A flexible outlier detector based on a topology given by graph communities

Outlier, or anomaly, detection is essential for optimal performance of machine learning methods and statistical predictive models. It is not just a technical step in a data cleaning process but a key topic in many fields such as fraudulent document detection, in medical applications and assisted diagnosis systems or detecting security threats. In contrast to population-based methods, neighborhood based local approaches are simple flexible methods that have the potential to perform well in small sample size unbalanced problems. However, a main concern of local approaches is the impact that the computation of each sample neighborhood has on the method performance. Most approaches use a distance in the feature space to define a single neighborhood that requires careful selection of several parameters. This work presents a local approach based on a local measure of the heterogeneity of sample labels in the feature space considered as a topological manifold. Topology is computed using the communities of a weighted graph codifying mutual nearest neighbors in the feature space. This way, we provide with a set of multiple neighborhoods able to describe the structure of complex spaces without parameter fine tuning. The extensive experiments on real-world data sets show that our approach overall outperforms, both, local and global strategies in multi and single view settings.

==> figs/graph.tex <==
 
\def\Pi{(0,0) ellipse (10mm and 3mm)} % Covariance of xhat_1
\def\el{ ellipse (10mm and 3mm) } % Covariance of xhat_2
\tikzstyle{P_1} = [draw,red,thick]
\tikzstyle{P_2} = [draw,blue,thick]

 \begin{tikzpicture}[line cap=round,line join=round]
    \tkzDefPoint(-2,5.5){A}
    \tkzDefPoint(7,2){B}
    \tkzDefPoint(8,2){C}
    
    % Axis
    \begin{axis}[
    axis equal,
    scatter/classes={%
    +={mark=+,draw=red},
    -={mark=o,draw=blue}},
    enlarge y limits={value=.1,upper},
    %   tick align=inside,
    %             height=5cm,     % size of the image
    ylabel=$p_{\ell_{\V}}^{con}$,
    xlabel=$\sigma_{\V}^{div}$,
    axis lines=middle,
    axis line style={->},
    x label style={at={(current axis.right of origin)},right=5mm},
    y label style={at={(current axis.above origin)},anchor=north, above=5mm},
    %         y axis line style={opacity=0}, 
    %         x=1.2cm,
    enlarge x limits={abs=0.5cm},
    legend style={
    at={(1.5,1)},
    % legend columns=-1,
    /tikz/every even column/.append style={column sep=0.5cm}
    },
    ]        
    
    \addplot[scatter,only marks,scatter src=explicit symbolic] table[x=x,y=y,meta=label]  {data/OutliersIris.txt};
    \legend{Positive samples, Outliers}
    \end{axis} 
   
    
    % \draw[-latex] (0,0) --(2.5,0);
    % \draw[-latex] (0,0) --(0,2.5);
    
    % \draw (2,0) -- (2,2) --(0,2);

    % Primera configuració
    \draw[red,thin,name path=elip] (A) \el;

    \pgfmathsetseed{24122015}
    \coordinate (p0) at ($ (A) + (.9,1mm) $);
    \fill[blue] (p0)  circle (0.05);
    \foreach \p in {1,...,10}
    {
        \coordinate (p\p) at ($ (A) + (rand,.2*rand) $);
        \fill[red] (p\p)  circle (0.05);
    }
    \draw[-latex] (p0) to [bend left=60]  (.5,5.5);
    \node at ($(A) + (0,-.5cm)$) {$\C_i$};

     
    \begin{scope}[rotate=-10]
        \draw[red,thin,name path=elip2] (B) \el;
        \coordinate (q0) at ($ (B) + (1mm,1mm) $);
        \foreach \q in {1,...,10}
        {
            \coordinate (q\q) at ($ (B) + (rand,.3*rand) $) ;
            \fill[red] (q\q)  circle (0.05);
        }
        % \foreach \q in {1,...,9}
        % {
        %     \draw (q\q) -- (q0);
        % }
    \end{scope}
    \begin{scope}[rotate=20]
        % \path[P_1] \Pi;
        \path[P_2] (C) \el;
        % \path (-1.5,0) node[left] {$\hat{x}_1$}
        %     (0,1.5) node [right] {$\hat{x}_2$};
        \coordinate (r0) at ($ (C) + (1mm,1mm) $);
        \foreach \r in {1,...,10}
        {
            \coordinate (r\r) at ($ (C) + (rand,.3*rand) $) ;
            \fill[blue] (r\r)  circle (0.05);
        }
        % \foreach \r in {1,...,9}
        % {
        %     \draw (r\r) -- (r0);
        % }
    \end{scope}


 

       
    \end{tikzpicture} 
